Context-Aware Replanning with Pre-explored Semantic Map for Object Navigation

Pre-explored Semantic Maps, constructed through prior exploration using visual language models (VLMs), have proven effective as foundational elements for training-free robotic applications. However, existing approaches assume the map's accuracy and do not provide effective mechanisms for revising decisions based on incorrect maps. To address this, we introduce Context-Aware Replanning (CARe), which estimates map uncertainty through confidence scores and multi-view consistency, enabling the agent to revise erroneous decisions stemming from inaccurate maps without requiring additional labels. We demonstrate the effectiveness of our proposed method by integrating it with two modern mapping backbones, VLMaps and OpenMask3D, and observe significant performance improvements in object navigation tasks. More details can be found on the project page: https://care-maps.github.io/

==> links.tex <==
% Po-Chen slides https://docs.google.com/presentation/d/1O-uGq5_qVp4Y3iMU_-_NvyKSB8mWLUiJDD3osTtRqdk/edit?usp=sharing

% Jeffrey Slide
% https://docs.google.com/presentation/d/16Rvae3FzoZK9F1c2XCDCHXA4ikUMb6wXefeci42cZ9E/edit?usp=sharing

==> sections/1_old_intro.tex <==
\section{Introduction}\label{sec:1:intro}
\htRevise{Object navigation, which involves localizing and navigating to an object in indoor environments, is a critical component of robotic applications.} 
Conventional training-based methods necessitate extensive annotations, meticulous model design, and prolonged training periods to effectively align the control actions with visual perception. 
Advancements in visual language models (VLMs) have led to the development of modular approaches that separate perception from actions, utilizing pre-trained knowledge. Under this framework, visual perception can be independently learned without direct control, making exploration prior to task execution an effective strategy. 
%\todo{cite some papers}
\map{} \cite{mapjatavallabhula2023conceptfusion,mapshafiullah2023clip,maptakmaz2023openmask3d,nlmapchen2023open,vlmapshuang2023visual}, constructed through prior exploration and using visual language models (VLMs), has become a fundamental backbone for robotics tasks. By constructing the map during environmental exploration, \map{} equips the agent with pre-existing knowledge of the environment, facilitating training-free robotic tasks such as manipulation motion planning \cite{huang2023voxposer}, interactive exploration \cite{jiang2024roboexp}, and zero-shot object navigation \cite{vlmapshuang2023visual}. 
However, current approaches presume \map{} is always accurate and lacks effective mechanisms for revising decisions based on incorrect maps. This assumption is incorrect for real-world applications, as visual perception must contend with varied environments featuring different lighting conditions, textures, weather, and dynamic elements. Consequently, visual perception cannot be assumed to be perfect. In addition, evaluating the quality of the \map{} is also challenging, as there are no existing labels for comparison.

Intuitively, the map-based agent plans its path by retrieving the goal from the map, where retrieval is facilitated by sorting confidence scores based on map-query matching. Therefore, should the initial attempt fail, the agent can proceed to another unvisited location with the highest confidence score. Nevertheless, this approach assumes the map is accurate. However, failure to retrieve the map with the highest confidence score may indicate a mismatch or error in the map-query alignment. Given the observation that the visual observation upon which the map is based fails to satisfy the query, we hypothesize that integrating \textbf{Uncertainty} measurement into the decision-making process can enhance the agent's ability to cope with inaccuracies in the map. By prioritizing areas with the greatest uncertainty, the agent targets high-uncertainty points for maximum information gain. This improves performance because initial prediction failures often result from biases or errors in the map data. Replanning based solely on confidence scores can perpetuate these biases. High-uncertainty areas, however, are less influenced by existing biases, providing new, unbiased information that can correct or enhance the agent’s understanding. Thus, integrating uncertainty measurement reduces bias impact and increases the likelihood of successfully finding the goal. In addition, the same region can be observed from multiple viewpoints. If the VLM predictions from these multiple viewpoints are not aligned, the prediction is likely incorrect. Therefore, \textbf{Multi-view Consistency} can also serve as an unsupervised metric for agent replanning.

\input{figures/fig1}
%By prioritizing exploration of areas with the greatest uncertainty or lowest confidence in the map’s accuracy, the agent identifies high-uncertainty points as indicators of where the maximum information gain can be achieved. This approach improves performance because it addresses the limitations observed when the top1 prediction fails. When the highest confidence region does not satisfy the query, it suggests that the agent's existing map data may be incorrect or incomplete. By exploring high-uncertainty areas among the top candidates, the agent is more likely to find a region that corrects or complements the initial prediction. This method leverages the assumption that areas of high uncertainty are critical for verifying or refuting the agent’s current knowledge, thus increasing the chances of success. Consequently, this strategy allows the agent to make more informed and reliable decisions by focusing on the areas that offer the most potential for correcting initial prediction errors, even without retraining the model.
%not only seeks to confirm or correct the existing map data but also 
%This method leverages the intuition that areas with higher uncertainty are likely to provide the most informative data for refining the map, thereby turning potential navigational errors into opportunities for improvement. This proactive approach to uncertainty ensures that the agent continuously adapts to new information, thereby enhancing its ability to navigate complex and dynamic environments more reliably. 

%map failure - visual perception not perfect
%modualize
To this end, we propose a novel \textbf{\ourmap{} (\ourmapabbr{})} to revise the plan when the initial planning fails. Specifically, we first select $k$ candidate regions as a strategy to mitigate the limitations of imperfect perception systems. While the top-ranked region might not always be reliable due to potential inaccuracies in perception, selecting a broader set of top candidates ensures a more robust assessment. Afterward, we measure uncertainty and multi-view consistency for candidate regions. For uncertainty, we sort the regions by the entropy of VLM predictions and select the highest. For multi-view consistency, we measure the average pair-wise KL-divergence and select the lowest. \ourmap{} is modular, portable to different backbones, and leverages the context of \map{} without requiring additional annotations. Consequently, \ourmap{} enhances decision-making resilience and, while focused on replanning, holds potential for continuous map refinement in future studies.
%we prioritize regions with incomplete or ambiguous map data, directing the agent to areas likely to benefit from further exploration. This method enhances decision-making resilience and, while focused on replanning, holds potential for continuous map refinement in future studies.
%replanning the agent based on the uncertainty of candidate regions. 
 %Second, 
 %we measure the uncertainty of candidates and replan the agent accordingly. Since \map{} is constructed using visual perception models from multiple viewpoints, we utilize the confidence scores and consistency across these views, thereby eliminating the need for additional annotations. Utilizing uncertainty, we prioritize regions with incomplete or ambiguous map data, directing the agent to areas likely to benefit from further exploration. This method enhances decision-making resilience and, while focused on replanning, holds potential for continuous map refinement in future studies.
%estimating the uncertainty of the \map{} 
%by measuring its confidence scores and multi-view consistency. We hypothesize that 
%When the agent failed to locate the goal following the map, \ourmap{} re-plan by exploring 

To demonstrate the modularity and robustness of \ourmapabbr{}, we conducted experiments using two \map{} backbones, VLMaps \cite{vlmapshuang2023visual} and OpenMask3D \cite{maptakmaz2023openmask3d}, showcased their effectiveness in object navigation tasks. The results demonstrate that \ourmapabbr{} consistently outperforms the strategy of selecting the highest-scored unvisited region. We tested two different strategies for measuring uncertainty: single-view confidence-based and multi-view consistency. Both approaches proved effective, validating our hypothesis that leveraging uncertainty improves the overall effectiveness of \map{}-based applications, with navigation serving as a prime example. Given its modularity and portability, we encourage future research to consider integrating \ourmapabbr{} into a broader range of robotic applications.

The contribution of this work is summarized as follow:
\begin{itemize}
\item We propose a novel \ourmap{} (\ourmapabbr{}), which replans based on the context of an incorrect \map{} when the initial task fails.
\item We design two variants of \ourmap{}, based on uncertainty and multi-view inconsistency, without requiring additional annotations.
\item Our method consistently outperforms the strategy of selecting the highest-scored unvisited region using two different backbones, VLMaps \cite{vlmapshuang2023visual} and OpenMask3D \cite{maptakmaz2023openmask3d}, demonstrating its effectiveness and robustness.
\end{itemize}

%\map{}, constructed through prior exploration, aids in indoor robotic tasks. However, current approaches presume \map{} is always accurate and lacks mechanisms for revising decisions based on incorrect maps.

%We propose an \ourmap{} that evaluates the accuracy of the constructed \map{} without labels, by assessing uncertainty through multi-view consistency and confidence measures.

%Leveraging \ourmap{}, we propose an entropy-based method to revise and replan object navigation strategies when initial tasks fail.

%Experimental results ... outperform ...


% \pcko{What I have (In openmask3d):
%     \begin{enumerate}
%         \item Some plots of different levels of uncertainty vs successes/failures. We can say something about why we care about uncertainty with these plots.
%         \item A quantitative table replanning with both single-view (entropy) and multi-view uncertainty measures (Feature variance and pairwise KL div). The table shows positive results on all these measures, but the single-view entropy-based replanning seems to work the best. 
%         The conclusion of this table is as below:
%         \begin{enumerate}
%             \item For single-view uncertainty metrics, the higher the better. (False beliefs of the map?)
%             \item For multi-view uncertainty metrics, the lower the better. (Multi-view consistency)
%         \end{enumerate}
%     \end{enumerate}
% What I plan to do: 
%     \begin{enumerate}
%         \item Try to combine single-view and multi-view measures to achieve even better performance. If this is successful we can extend the table above and say more about the benefits of fusing different uncertainty metrics in our article. If this is not successful we can discuss more about how to present the table later on. (At least we want to show the single-view results because it works well in both om3d and vlmaps, but for multi-view results, maybe we can consider putting them in the appendix)
%     \end{enumerate}
% }
